Linear MHD stability studies with the STARWALL code

The STARWALL/CAS3D/OPTIM code package is a powerful tool to study the linear MHD stability of 3D, ideal equilibria in the presence of multiply-connected ideal and/or resistive conducting structures, and their feedback stabilization by external currents. Robust feedback stabilization of resistive wall modes can be modelled with the OPTIM code. Resistive MHD studies are possible combining STARWALL with the linear, resistive 2D CASTOR code as well as nonlinear MHD simulations combining STARWALL with the JOREK code. In the present paper, a detailed description of the STARWALL code is given and some of its applications are presented to demonstrate the methods used. Conducting structures are treated in the thin wall approximation and depending on their complexity they are discretized by a spectral method or by triangular finite elements. As an example, a configuration is considered consisting of an ideal plasma surrounded by a vacuum domain containing a resistive wall and bounded by an external wall. Ideal linear MHD modes and resistive wall modes in the presence of multiply-connected walls are studied. In order to treat the vertical mode self-consistently the STARWALL code has been completed by adding the so-called Luest-Martensen term generated by a constant normal displacement of the plasma. The appendix contains the computation of the 2D Fourier transform of singular inductance integrals, and the derivation of an asymptotic expansion for large Fourier harmonics.

==> bibmacp.tex <==
% create item in bibliography by
%                        \addbibitem {\name} {text}
% citation by name like this
%                        \cite{\name}
%
\newcount\bibnum
\bibnum = 0
\newbox\bibtext
\setbox\bibtext=\vbox{}
\newdimen\bibsize
\bibsize=0pt
%
\def\bibwrite{\unvbox\bibtext}
%
\def\addbibitem #1 #2{\global\advance\bibnum by 1
\xdef#1{\the\bibnum}
\global\setbox\bibtext=\vbox{\unvbox\bibtext%
\tolerance=10000 \hbadness=8000 \begingroup \parindent=0.55truecm\medpoint
%\tolerance=10000 \hbadness=8000 \begingroup \parindent=0.55truecm
\item{\hbox to \parindent{\hfill\lb \the\bibnum \rb}}#2 \par
%\medskip \endgroup }}
\endgroup }}
\def\bibskip{\medskip}
%\def\cite#1{$^{#1}$}
\def\cite#1{\lb #1\rb}
\def\onlinecite#1{#1}


==> citations.tex <==
{\bf CITATIONS}
\par
\bigskip
$\bullet$ {\sl Resistive wall modes of 3D equilibria with multiply-connected 
walls \cite{Merkel2004}}
\par
STARWALL code
\par
\bigskip
$\bullet$ {\sl Resistive wall modes of 3D equilibria with multiply-connected
walls \cite{Merkel2006}}
\par
STARWALL code
\par
\bigskip
$\bullet$ {\sl On fully three-dimensional resistive wall mode and feedback
stabilization computations \cite{Strumberger2008}}
\par
results for ITER and AUG; toroidal mode coupling may be insignificant 
for ITER wall; holes in the wall lead to a considerable increase of
the groth rate for both, ITER and AUG; the complex structure of the
AUG wall design leads to a significant coupling of the toroidal harmonics;
feedback stabilization;
\par
\bigskip
$\bullet$ {\sl Three-dimensional effects in tokamaks \cite{Guenter2008}}
\par
Benchmark of STARWALL with CASTOR-FLOW, MARS, VALEN and KINX codes;
\par
\bigskip
$\bullet$ {\sl Robust control of resistive wall modes using pseudospectra
\cite{Sempf2009}}
\par
OPTIM code, ITER example
\par
\bigskip
$\bullet$ {\sl In-vessel saddle coils for MHD control in ASDEX Upgrade
\cite{Suttrop2009}}
\par
RWM control; AUG example
\par
\bigskip
$\bullet$ {\sl Linear stability studies in the presence of 3D wall structures 
\cite{Strumberger2011}}
\par
STARWALL/OPTIM calculations for AUG example; extension of CASTOR$\_$FLOW
to CASTOR$\_$3DW and coupling with the STARWALL code;
\par
\bigskip
$\bullet$ {\sl Recent ASDEX Ugrade results and future extension plans 
\cite{Kallenbach2012}}
\par
Growth rates as function of $\beta_N$ for different wall coverage scenarios
(with ICRF antennas).
\par
\bigskip
$\bullet$ {\sl Coupling JOREK and STARWALL codes for non-linear resistive-wall
simulations \cite{Freidberg1989}}          
\par
\bigskip 
$\bullet$ {\sl Coupling JOREK and STARWALL codes for non-linear resistive-wall
simulations \cite{Merkel1986}}          
 \cite{Hirshman1_1986}          
 \cite{Hirshman1983}          
 \cite{Chu2010}          
 \cite{Kameari1981}          
 \cite{OKAMURA2001}          
 \cite{Nuehrenberg1996}          
 \cite{Bialek2001}          
 \cite{Bialek2007}          
 \cite{Chu2003}          
 \cite{Portone2008}          
 \cite{Villone2008}          
 \cite{Liu2004}          
 \cite{Nuehrenberg1987}          
 \cite{Merkel1987}          


==> singulint.tex <==
\par
\medskip
$$
K_{mn}=\pi\int\limits_0^1\int\limits_0^1\,du\,dv\,
{(A\tan^2(\pi u)+2B\tan(\pi u)\tan(\pi v)+C\tan^2(\pi v))
e^{2\pi i(mu+nv)}\over
(a\tan^2(\pi u)+2b\tan(\pi u)\tan(\pi v)+
c\tan^2(\pi v))^{3\over2}}
\eqno (A2)
$$
with $ac - b^2 > 0 $.
The integrals $K_{mn}$ can be derived from the integrals
$I_{mn}$ by differentiation:
$$
K_{mn}=-2(A{\partial\over \partial a}+B{\partial\over
\partial b}+C{\partial\over \partial c})I_{mn}\,.
$$
To compute the $I_{mn}$ a generating function $I$ is
introduced:
$$
I=\sum\limits_{m=0,n=0}^{\infty ,\infty}
I_{mn}s^mt^n\,.
$$
Summing up the power series, one obtains $I$ in
closed form:
$$
I=\pi\int\limits_0^1\int\limits_0^1
{du\,dv \over (1-se^{2\pi iu})(1-te^{2\pi iv})
(a\tan^2(\pi u)+2b\tan(\pi u)
\tan(\pi v)+c\tan^2(\pi v))^{1\over2}}.
$$
Introducing new variables $r, y$
$$
y = \tan \pi u\,
ry= \tan \pi v\,
$$
one gets for $I$
$$
I = {1 \over 4\pi} \int\limits_{-\infty}^{+\infty}
\int\limits_{-\infty}^{+\infty}
\,dr\,dy\,\biggl( {1 \over y+i\alpha}-{1 \over y-i}
\biggr) \biggl( {1 \over ry+i\beta} - {1 \over ry-i}
\biggr) {1 \over (a+2br+cr^2)^{1 \over 2}}
$$
with
\begin{eqnarray*}
\alpha &= {1-s \over 1+s}\\ 
\beta &= {1-t \over 1+t} .
\end{eqnarray*}
Integrating $I$ with respect to $y$, one obtains
\begin{eqnarray*}
 I &=& {1 \over 2} \int\limits_0^\infty\,dr
\biggl( {1 \over \beta +\alpha r} + {1 \over 1+r}
\biggr) {1 \over (a-2br+cr^2)^{1 \over 2}} \\
&+& {1 \over 2} \int\limits_0^\infty\,dr
\biggl( {1 \over 1+\alpha r} + {1 \over \beta +r}
\biggr) {1 \over (a+2br+cr^2)^{1 \over 2}}\,.
\end{eqnarray*}
\begin{eqnarray*}
   \int\limits_0^\infty\,dr
\biggl( {1 \over \beta +\alpha r}
\biggr) {1 \over \sqrt{a-2br+cr^2}} &=&
   \frac{1}{\gamma} \ln{\frac{\alpha(\gamma \sqrt{c} +\alpha c + 
  \beta b)}{\beta (\gamma \sqrt{a} -\alpha b - \beta a)}} 
\end{eqnarray*}
with $\gamma = \sqrt{a \beta^2 + 2 b \alpha \beta +c \alpha^2}$

If the integration variable $x = (1-r)/(1+r)$ is introduced
and $\alpha$ and $\beta$ are again expressed by $s$ and $t$,
the function $I$ can be written as a sum of four terms:
$$
I = h^+(s,t)+h^+(0,0)+h^-(s,0)+h^-(0,t)\,,
$$
where the function $h$ is defined by
$$
h^\pm (s,t)={(1+s)(1+t) \over 2}\,
\int\limits_{-1}^{+1}\,{dx \over (1-st-(s-t)x)
(a^\mp +2dx+a^\pm x^2)^{1 \over 2}}
$$
and the coefficients are given by
\begin{eqnarray*}
a^+ &=& a+2b+c, \\
a^- &=& a-2b+c, \\
d &=& c-a  .
\end{eqnarray*}
The final step in calculating the $I_{mn}$ is to expand
$I$ again as a power series in $s$ and $t$. One starts
by expanding the function $h$
$$
h^\pm (s,t)={1 \over 2}
{(1+s)(1+t) \over 1-st} \sum\limits_{\ell =0}^\infty
\biggl( {s-t \over 1-st}\biggr)^\ell T_\ell ^\pm
$$
with
$$
T_\ell ^\pm = \int\limits_{-1}^{+1}\,dx\,
{x^\ell \over (a^\mp+2dx+a^\pm x^2)^{1 \over 2}}
$$
Expanding $h$ further, one finally obtains for the
coefficients $I_{mn}$
\begin{eqnarray*}
I_{mn}=\left\{\begin{array}{*{3}{c@{+}}c@{,}c} 
 c^+_{m\,n} &c^+_{m-1\,n} &c^+_{m\,n-1} &c^+_{m-1\,n-1}&
{\rm for}\, m\ge 1,n\ge 1\\
c^+_{m\,0} &c^+_{m-1\,0} &c^-_{m\,0} &c^-_{m-1\,0}&
{\rm for}\, m\ge 1,n=0\\
c^+_{0\,n} &c^+_{0\,n-1} &c^-_{0\,n} &c^-_{0\,n-1}&
{\rm for}\, m=0,n\ge 1\\
c^+_{0\,0} &c^+_{0\,0} &c^-_{0\,0} &c^-_{0\,0}&
{\rm for}\, m=0,n=0\end{array} \right.
\end{eqnarray*}
with
$$
c^\pm_{mn}=\sum\limits_{\ell =0}^{{m+n-\vert m-n\vert \over 2}}
{(-1)^{\ell +{\vert m-n\vert -m+n \over 2}}
\bigl({m+n+\vert m-n\vert
\over 2}+\ell \bigr) !\,  T_{\vert m-n\vert +2\ell}^\pm
\over 2 \bigl({m+n-\vert m-n\vert \over 2}-\ell \bigr) !
(\vert m-n\vert +\ell)! \ell !}\,.
$$
The functions $T_\ell ^\pm$ defined in eq.(A12) can be
calculated by using a recurrence relation. Expressing the
coefficients $a^+, a^-, d$ by $a, b, c$ one
obtains
\begin{eqnarray*}
T_0^\pm & = &{1 \over \sqrt{a\pm 2b+c}}\log
{\sqrt {c(a\pm 2b+c)}+c\pm b \over
\sqrt {a(a\pm 2b+c)}-a\mp b}, \\
T_1^\pm &= &{1 \over {a\pm 2b+c}}
\bigl( 2(\sqrt c -\sqrt a)-(c-a)T_0^\pm \bigr), \\
T_\ell ^\pm &= &{1 \over {\ell (a\pm 2b+c)}}
\bigl( 2(\sqrt c +(-1)^\ell \sqrt a) \\
& - & (2\ell -1)(c-a)T_{\ell -1}^\pm -(\ell -1)
(a\mp 2b+c)T_{\ell -2}^\pm\bigr)\quad
{\rm for}\  \ell \ge 2\,.
\end{eqnarray*}
The Fourier integrals $K_{mn}$ follow from the $I_{mn}$
by differentiation (see eq.(A3)). For
the $K_{mn}$ one gets the same formulas, (A13), (A14), as for
the $I_{mn}$; only the integrals $T_\ell ^\pm$ have
to be replaced by integrals $S_\ell ^\pm$, which are
given by
$$
S_\ell ^\pm = \int\limits_{-1}^{+1}\,dx\,x^\ell\,
{(A^-+2D\,x+A^+x^2) \over (a^-+2d\,x+a^+x^2)^{3 \over 2}}
$$
with
\begin{eqnarray*}
A^+ &=& A+2B+C, \\
A^- &=& A-2B+C, \\
D &=& C-A \ .
\end{eqnarray*}
As for the $T_\ell ^\pm$, recurrence formulas can be derived
for the $S_\ell ^\pm$, but the $S_\ell ^\pm$ can also be
expressed in terms of the $T_\ell ^\pm$ by appropriate partial
integration. One obtains for $S_\ell ^+$
\begin{eqnarray*}
(a+2b+c)& &(ac-b^2)S_\ell ^+ =\\
& &\biggl( (A+2B+C)(ac-b^2)+\ell \bigl( k_1(a+2b+c)+k_2(c-a)
\bigr) \biggr)\,T_\ell ^+ \\
&+&\ell \bigl(k_1(c-a)+k_2(a-sb+c) \bigr)\,T_{\ell -1}^+ \\
&-& {(c+b)k_1+(c-b)k_2 \over \sqrt c}\,-\,(-1)^\ell\,
{(a+b)k_1-(a-b)k_2 \over \sqrt a}  
\end{eqnarray*}
with
\begin{eqnarray*}
k_1 &=& (a+c)B-(A+C)b, \\
k_2 &=& C(a+b)-B(c-a)-A(c+b). 
\end{eqnarray*}
The formula for $S^- _\ell$ is obtained by replacing
$b$ by   $-b$ and $B$ by   $-B$, and $T^+ _\ell , T^+ _{\ell -1}$
with $T^- _\ell , T^- _{\ell -1}$.
\par
For large $m$ and $n$ an asymptotic expansion can be derived
for the Fourier integrals $I_{mn}$ and $K_{mn}$.
For $ac - b^2 > 0 $
the leading terms are  \lbrack 21\rbrack
\begin{eqnarray*}
I_{mn} &=& {1 \over (an^2-2bnm+cm^2)^{1 \over 2}} \,,\\
K_{mn} &=& {An^2-2Bnm+Cm^2 \over (an^2-2bnm+cm^2)^{3 \over 2}}
\,.
\end{eqnarray*}

